RTSDF: Real-time Signed Distance Fields for Soft Shadow Approximation in Games

Signed distance fields (SDFs) are a form of surface representation widely used in computer graphics, having applications in rendering, collision detection and modelling. In interactive media such as games, high-resolution SDFs are commonly produced offline and subsequently loaded into the application, representing rigid meshes only. This work develops a novel technique that combines jump flooding and ray tracing to generate approximate SDFs in real-time. Our approach can produce relatively accurate scene representation for rendering soft shadows while maintaining interactive frame rates. We extend our previous work with details on the design and implementation as well as visual quality and performance evaluation of the technique.

==> relatedwork.tex <==
\section{\uppercase{Related Work}}

% \subsection{SDF}

% \subsubsection{Uniform SDF}

% Recently, \citet{krayer_muller_2019} has managed to generate SDFs on the GPU by first creating a distance transform based on the linear time algorithm by \citet{felzenswalb_2012}. The distance transform is simply an unsigned distance field. Subsequently, SDFs are generated using a ray map data structure that stores ray intersection information originating at each point in the map.

% A similar problem to calculating distance fields is generating Voronoi diagrams, which are partitionings of space into regions based on distances to a specific set of points which lie in the space. These points are generally referred to as seeds. Given that we know the closest seed to a point, we can calculate its distance to that seed in constant time. If we iterate for all points in the space, we will generate the distance transform. \citet{sud_otaduy_manocha_2004} uses hardware-accelerated rasterization to convert 3-dimensional primitives into a distance field. Notably, \citet{rong_tan_2006} has developed a logarithmic time algorithm known as jump flooding that can be executed in parallel on the GPU to approximate the distance fields. 

%  \begin{figure}[!h]
%      \centering
%      \includegraphics[width=\linewidth]{FIGURE/holes-in-surface.png}
%      \caption{Distance fields of different resolution.}
%      \label{fig:holes-in-surface}
%  \end{figure}

% Naturally, as the resolution of the 3D texture decreases, the number of samples reduces, giving a less accurate surface representation. This also becomes problematic for thin surfaces where a sample point does not lie within the enclosed surface, resulting in holes in the surface as illustrated in \autoref{fig:holes-in-surface}. With the low resolution (left), the inner portion of the surface is not saved. During interpolation between sample points, a negative value cannot be re-obtained. \citet{wright_2015} points out that these holes are not problematic for approximating sky occlusion, but will cause holes in the umbra of area light shadows. To circumvent this issue, a higher sampling frequency is required as shown. Alternatively, \citet{wright_2015} uses cascaded shadow maps instead for the umbra.

% \subsubsection{Adaptively Sampled Distance Field}

% Alternatively, as shown in \autoref{fig:adf}, SDFs can be stored in a hierarchical fashion as adaptively sampled distance fields \citep{frisken_perry_rockwood_jones_2000}, which has since been adapted by \citet{koschier_2016} and \citet{liu_kim_2014}. The goal is to reduce the memory footprint of storing highly-detailed SDFs. In these methods, spatial subdivision into octrees is carried out and the subdivision criteria is based the reconstruction error at the current level of subdivision.

%  \begin{figure}[!h]
%      \centering
%      \includegraphics[width=\linewidth]{FIGURE/ADF.PNG}
%      \caption{A hierarchical distance field. Source: \citet{frisken_perry_rockwood_jones_2000}.}
%      \label{fig:adf}
%  \end{figure}

% Regions with high level of detail are subdivided further for greater precision, allowing for a smaller memory footprint as empty regions are stored as single values. Additionally, this subdivision also provides a way to generate level-of-detail models like in \citet{frisken_perry_rockwood_jones_2000} where the octree is truncated based on the error. However, a disadvantage is the requirement to traverse the octree when raymarching, resulting in multiple memory accesses to read the final signed distance. In rendering, raymarching operations require multiple samples of the distance field and hence performance will be slowed down. Additionally, as noted by \cite{liu_kim_2014}, a tree representation is problematic for GPUs due to dynamic memory allocation and pointer creation. This also makes generating these distance fields every frame expensive for real-time rendering. For their game Claybook, \cite{aaltonen} measured the performance of a virtual indirection texture for sparse volumes and recorded a 13\% hit to performance.
